The importance of being dissimilar in Recommendation

Similarity measures play a fundamental role in memory-based nearest neighbors approaches. They recommend items to a user based on the similarity of either items or users in a neighborhood. In this paper we argue that, although it keeps a leading importance in computing recommendations, similarity between users or items should be paired with a value of dissimilarity (computed not just as the complement of the similarity one). We formally modeled and injected this notion in some of the most used similarity measures and evaluated our approach showing its effectiveness in terms of accuracy results.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> src/related.tex <==
%%%%%Several collaborative filtering methods have been developed and proposed in literature to address the recommendation problem. Although there have been many variations, the basic common idea is to compute similarity among users(user-based) or items(item-based) in order to recommend items based on this similarity measures. However the majority of the proposed similarity measures are symmetric meaning that the similarity between two users is the same for both. In the following we show state of art of both the symmetric similarity measures and the asymmetric ones. Among the symmetric similarity measures the most commonly used are the cosine similarity \cite{adomavicius2005toward}(RIVEDERE CIT), the Jaccard similarity\cite{candillier2008designing}(RIVEDERE CIT) and the Pearson correlation\cite{resnick1994grouplens}. 
%%%%%
%%%%%Before focusing on the recommendation approach the concept of similarity needs more attention.
%%%%%Several different similarity measures have been proposed and adopted for recommender systems:
%%%%%\begin{itemize}
%%%%%	\item Cosine Vector similarity (CV)\cite{DBLP:journals/cacm/BalabanovicS97}\cite{DBLP:journals/umuai/BillsusP00}\cite{abiteboul1995news}
%%%%%	\item Pearson Correlation similarity (PC or CORR)\cite{DBLP:journals/ir/HerlockerKR02}
%%%%%	\item Constrained Pearson correlation similarity\cite{DBLP:conf/chi/ShardanandM95}
%%%%%	\item Adjusted Cosine similarity (AC)\cite{DBLP:conf/www/SarwarKKR01}
%%%%%	\item Mean Squared Difference similarity (MSD)\cite{DBLP:conf/chi/ShardanandM95}
%%%%%	\item Spearman Rank Correlation (SRC)\cite{kendall1990rank}
%%%%%	\item Frequency-Weighted Pearson Correlation (FWPC)\cite{DBLP:conf/uai/BreeseHK98}
%%%%%	\item Target item weighted Pearson Correlation ($WPC_j$)\cite{DBLP:series/sci/BaltrunasR09}
%%%%%	\item Jaccard similarity\cite{dong2011efficient}\cite{qamar2008similarity}
%%%%%\end{itemize}
%%%%%The choice of the elected similarity to use usually depends on the specific scenario, available data and aspects of similarity that should be stressed.

%The cosine similarity looks at the angle between two vectors by measuring the cosine of that angle so that the smaller is the angle the greater is the similarity. However it should be noticed that there exist both an explicit and implicit feedback variant. On the other hand the Pearson correlation is used to measure the linear correlation between two vector of ratings. The Jaccard similarity instead measures the overlap between two vectors meaning that although two users rated the same items but with really different opinions it will give always an high similarity value. For this reason it is usually used in combination with other similarities that takes into account ratings such as the Pearson correlation. However in real word situations it is really difficult to have explicit feedback since it requires a user more effort. This is the reason why we are inspecting in our approaches only similarities that take advantage of implicit feedback. Other similarities have been developed in order to deal with some of the drawbacks of the previously mentioned similarities such as the adjusted cosine similarity\cite{sarwar2001item}(RIVEDERE CIT) that differently from the cosine considers that different users can have a different rating scale, the constrained Pearson Correlation(there are also other variants such as SPCC, WPCC) that uses the median value in the rating scale instead of the average rating of a user for all the co-rated items(in order to consider the impact of positive and negative ratings) or the Spearman rank correlation\cite{govindarajulu1992rank} that considers the ranking of the ratings instead of their values. More recently other similarity measures are emerging such as the new  heuristic similarity model(NHSM)\cite{liu2014new} that considers that different users have different rating preferences by using the mean and the variance of the rating.(CITARNE ALTRE?)
%
%Finally in literature very few works that use the concept of asymmetric similarities have been made and all of them investigated only the user-based variant. In \cite{millan2007collaborative} the authors underline that a similarity measure should make a distinction when a user has a lot more historical information than another one. In order to do that they made a small change at the Jaccard index in order to consider only the number of ratings of the current user and not that of both user. In \cite{katarya2016effectivecollaborative} and \cite{pirasteh2015exploiting} they multiplied the previous work similarity with the Sorensen index (that is not so different from the Jaccard index). Than they also multiplied this value for a similarity measure based on ratings but we are not interested in it since our approaches have been developed to deal with implicit feedbacks. However all this works evaluated the prediction quality of their methods just by using accuracy metrics such as RMSE and MAE.
%
%
%In \cite{pirasteh2015exploiting} they also factorize a user-user matrix containing the similarities previously computed in order to predict the missing values.
%In \cite{katarya2016effectivecollaborative} they create a computational expensive system called HYBRTyco where they combine factorization technique with an asymmetric model for similarity and typicality-based collaborative filtering.


%the Proximity, Impact, Popularity similarity used to overcome the weakness of traditional similarity measures in user cold-start condition

